Up-and-Down and the Percentile-Finding Problem

Up-and-Down (U&D) is a popular sequential design for estimating threshold percentiles in binary experiments. However, U&D application practices have stagnated, and significant gaps in understanding its properties persist. The first part of my work aims to fill gaps in U&D theory. New results concerning stationary distribution properties are proven. A second focus of this study is nonparametric U&D estimation. An improvement to isotonic regression called "centered isotonic regression" (CIR), and a new averaging estimator called "auto-detect" are introduced and their properties studied. Bayesian percentile-finding designs, most notably the continual reassessment method (CRM) developed for Phase I clinical trials, are also studied. In general, CRM convergence depends upon random run-time conditions -- meaning that convergence is not always assured. Small-sample behavior is studied as well. It is shown that CRM is quite sensitive to outlier sub-sequences of thresholds, resulting in highly variable small-sample behavior between runs under identical conditions. Nonparametric CRM variants exhibit a similar sensitivity. Ideas to combine the advantages of U&D and Bayesian designs are examined. A new approach is developed, using a hybrid framework, that evaluates the evidence for overriding the U&D allocation with a Bayesian one.

==> diss_intro_1.tex <==
\section{Overview and Definition of the Problem}
In many binary-response experiments, researchers are not interested in finding the entire treatment-response curve, but only a single representative value, which can be described via a percentile of the underlying threshold distribution $F$. This percentile can represent (for example) the sensory threshold, the $LD_{50}$ of a toxic substance, or the maximum-tolerated-dose (MTD) of a medication. Such experiments are typically performed under sample-size constraints, and with little prior knowledge about the form of $F$. An additional, rather common constraint is that treatment levels are limited to a discrete finite set.

Statisticians have been developing designs to answer this type of challenge for at least two generations. Yet, interestingly, if an applied researcher were to seek statistical consulting on this problem, he or she would receive wildly differing recommendations, depending upon which statistician happened to be the consultant. Moreover, an applied statistician wishing to consult a client on this issue would discover, upon a cursory literature search, that any clear, well-tested and practical guidelines (if they exist) are drowning in a sea of open questions, unbased claims and controversy.
These are not hypothetical statements; this is exactly what happened to me in late 2003, when attempting to help Dr. M. J. Souter design a percentile-finding experiment \citep{Oron2004}. Over the next years, my search for solid and reliable design solutions has evolved into the dissertation you are reading.

After this tortuous journey, I find it important to repeat in this introduction a well-known truism, which is somehow forgotten in this field's prevalent patterns of debate:

Constrained by the binary response, a small sample size, an unknown distribution function and a discrete treatment set, the quality of information (i.e. estimates) the experiment can provide is limited. Failed experiments (however one chooses to define 'failure') are far from unlikely. The degree of confidence expressed by many statisticians promoting this or that method is exaggerated. Keeping this perspective in mind, there is quite enough room for theoretical insight and methodological developments. 

The following tome focuses on the most veteran family of designs, a.k.a. 'Up-and-Down' (U\&D): Chapter 2 tackles the designs themselves, while Chapter 3 is devoted to estimation. The Bayesian Continual Reassessment Method (CRM), which has quickly eclipsed U\&D in the number of statisticians swearing by it, is discussed in Chapter 4. Many researchers point to the relationship between the two approaches, via definitions like the one below.

The definition is in the spirit of \cite{IvanovaFlournoy06} and others.
\begin{defn} (i) An {\bf 'Up-and-Down' design} is any percentile-finding, binary-outcome sequential experimental design with treatments and responses $\{x_n\},\{z_n\}$, respectively; with fixed, discrete treatment levels $\{l_m\}$ and sequential transition rules.

(ii) In an {\bf algorithmic or nonparametric U\&D design}, the transition rules are functions of $\{x_n\},\{z_n\}$ and possibly also $\phi$, a set of fixed parameters.

(iii) In a {\bf model-based or parametric U\&D design}, the transition rules are functions of $\{x_n\},\{z_n\}, \phi$, and a statistical model $f\left(\{x_n\},\{z_n\}\mid\theta\right)$, where $\theta$ is a set of data-estimable parameters.
\end{defn}

U\&D, of course, is an algorithmic/nonparametric design approach, and CRM a model/parametric one. 

There has been some attempts to combine the two, and I have devoted quite a bit of energy doing this. Combined approaches are dicussed in Chapter 5, which is followed by the conclusions.

Each Chapter begins with an introductory section, which reviews the current state of knowledge on the chapter's topic.



